The Ant Swarm Neuro-Evolution Procedure for Optimizing Recurrent Networks

Hand-crafting effective and efficient structures for recurrent neural networks (RNNs) is a difficult, expensive, and time-consuming process. To address this challenge, we propose a novel neuro-evolution algorithm based on ant colony optimization (ACO), called ant swarm neuro-evolution (ASNE), for directly optimizing RNN topologies. The procedure selects from multiple modern recurrent cell types such as Delta-RNN, GRU, LSTM, MGU and UGRNN cells, as well as recurrent connections which may span multiple layers and/or steps of time. In order to introduce an inductive bias that encourages the formation of sparser synaptic connectivity patterns, we investigate several variations of the core algorithm. We do so primarily by formulating different functions that drive the underlying pheromone simulation process (which mimic L1 and L2 regularization in standard machine learning) as well as by introducing ant agents with specialized roles (inspired by how real ant colonies operate), i.e., explorer ants that construct the initial feed forward structure and social ants which select nodes from the feed forward connections to subsequently craft recurrent memory structures. We also incorporate a Lamarckian strategy for weight initialization which reduces the number of backpropagation epochs required to locally train candidate RNNs, speeding up the neuro-evolution process. Our results demonstrate that the sparser RNNs evolved by ASNE significantly outperform traditional one and two layer architectures consisting of modern memory cells, as well as the well-known NEAT algorithm. Furthermore, we improve upon prior state-of-the-art results on the time series dataset utilized in our experiments.

==> acknowledgement.tex <==
\section*{Acknowledgement}
Most of the computation of this research was done on the high performance computing clusters of Research Computing at Rochester Institute of Technology. We thank the Research Computing team for the assistance and the support they generously offered to let this work see the light.

==> app_01.tex <==
\section{Ant Colony Algorithm}
\input{031-aco_pesudo_code.tex}

==> app_02.tex <==
\section{Fitness Structure Coefficient}
    Figure~\ref{fig:fit_strct_coeff} examines the relationship between the size of the network and its fitness. Results for RNNs from the top ten best performing experiments are shown along with \nn from the individual heuristic experiments.

    The following equation was used to calculate a measure of the contribution of each weight to the fitness of the RNN:

    \begin{equation}
        \label{eq:fit_strct_coeff}
        C_{fit\_struct} = \frac{1-MAE}{W_S}
    \end{equation}

    where $C_{fit}$ is a structural coefficient calculated by $MAE$, the mean absolute error of the RNN, and $W_S$, the number of weights in in that RNN structure. Higher values represent RNNs where weights contribute more to the performance of the network. 
    
    \begin{figure}[h]
		    \centering
		    \includegraphics[angle=-90,origin=c,width=.98\textwidth, height=.55\textheight]{./pix/{fit_strct_coeff_withSolo.pdf}}
		    \caption{Ranges of how much each weight in an RNN contributed to its performance (Equation~\ref{eq:fit_strct_coeff}). }
		    \label{fig:fit_strct_coeff}
	    \end{figure}

==> memory_cell_equations.tex <==

            \begin{equation}\label{eqs:lstm}
                \begin{gathered}
                    f = \sigma(W_f*x + U_f*c_prev * f_bias)     \\
                    i = \sigma(W_i*x + U_i*c_prev * i_bias)     \\
                    o = \sigma(W_o*x + U_o*c_prev * o_bias)     \\
                    c = f * c_prev + i * tanh(W_c*x + c_bias)   \\
                    h = o*c 
                \end{gathered}
            \end{equation}
            where $x$: input,
                  $h$: output,
                %   $W_f$: input forget-gate weights,
                %   $U_f$: previous cell memory forget-gate weights,
                %   $W_i$: input input-gate weights,
                %   $U_i$: previous cell memory input-gate weights,
                %   $W_o$: input output-gate weights, and
                %   $U_o$: previous cell memory out-gate weights
        
    
            \begin{equation}\label{eqs:gru}
                \begin{gathered}
                    z = \sigma(zw*x + zu*h_prev * z_bias)   \\
                    r = \sigma(rw*x + lu*h_prev * r_bias)   \\
                    k = hw*x + hu*r*h_prev * h_bias         \\
                    h = z*h_prev + (1-z)* tanh(k)
                \end{gathered}
            \end{equation}
            where $x$: input,
                  $h$: output,
                	
                	
            \begin{equation}\label{eqs:mgu}
                \begin{gathered}
                    f = \sigma(fw*x + fu*h_prev * f_bias)   \\
                    h = tanh(hw*x + f*hu*h_prev * h_bias)   \\
                    out = (1-f)*h_prev + f*h
                \end{gathered}
            \end{equation}
            where $x$: input,
                  $h$: output,
            
            \begin{equation}\label{eqs:ugrnn}
                \begin{gathered}
                    c = tanh(cw*x + ch*h_prev * c_bias) \\
                    g = \sigma(gw*x + gh*h_prev * g_bias)    \\
                    h = g*h_prev + (1-g)*c
                \end{gathered}
            \end{equation}
            where $x$: input,
                  $h$: output,
            
            
            \begin{equation}\label{eqs:delta}
                \begin{gathered}
                    \hat h_1 = \alpha*(v*h_{prev})*x    \\
                    \hat h_2 = \beta_1*v*h_{prev} + \beta_2*x          \\
                    % \hat h_3 = \beta_2*x                \\
                    \bar h = tanh(\hat h_1 + \hat h_2 + bias_{\hat h} )             \\
                    r = \sigma(x + bias_r)                  \\
                    h = tanh\Big((1-r)*\bar h + r*h_{prev}\Big)
                \end{gathered}
            \end{equation}
            where $x$: input,
                  $h$: output,
        
        
        
        	\begin{figure}
        	    \centering
        		\subfloat[LSTM Cell\label{fig:lstm}]{%
        			\centering
        			\includegraphics[width=.68\textwidth, height=.15\textheight]{./pix/{lstm_graph.pdf}}
        			}
        			\\
        		\subfloat[GRU Cell\label{fig:gru}]{%
        			\centering
        			\includegraphics[width=.68\textwidth, height=.15\textheight]{./pix/{gru_graph.pdf}}
        			}
        			\\
        		\subfloat[MGU Cell\label{fig:mgu}]{%
        			\centering
        			\includegraphics[width=.68\textwidth, height=.15\textheight]{./pix/{mgu_graph.pdf}}
        			}
        		    \\
        		\subfloat[UGRNN Cell\label{fig:ugrnn}]{%
        			\centering
        			\includegraphics[width=.68\textwidth, height=.15\textheight]{./pix/{ugrnn_graph.pdf}}
        			}
        			\\
        		\subfloat[$\Delta$-RNN Cell\label{fig:delta}]{%
        			\centering
        			\includegraphics[width=.68\textwidth, height=.15\textheight]{./pix/{delta_graph.pdf}}
        			}
        		\caption{RNN Memory Cells}
        		\label{fig:memory_cells}
        	\end{figure}

    	
